Can You Read Me Now? Content Aware Rectification using Angle Supervision

The ubiquity of smartphone cameras has led to more and more documents being captured by cameras rather than scanned. Unlike flatbed scanners, photographed documents are often folded and crumpled, resulting in large local variance in text structure. The problem of document rectification is fundamental to the Optical Character Recognition (OCR) process on documents, and its ability to overcome geometric distortions significantly affects recognition accuracy. Despite the great progress in recent OCR systems, most still rely on a pre-process that ensures the text lines are straight and axis aligned. Recent works have tackled the problem of rectifying document images taken in-the-wild using various supervision signals and alignment means. However, they focused on global features that can be extracted from the document's boundaries, ignoring various signals that could be obtained from the document's content. We present CREASE: Content Aware Rectification using Angle Supervision, the first learned method for document rectification that relies on the document's content, the location of the words and specifically their orientation, as hints to assist in the rectification process. We utilize a novel pixel-wise angle regression approach and a curvature estimation side-task for optimizing our rectification model. Our method surpasses previous approaches in terms of OCR accuracy, geometric error and visual similarity.

==> 51_textract_ref.tex <==
The vast majority of recent OCR methods are targeted at scene-text, with the number of proposed text instance detections often limited to 100-200. Thus, they are not suited to handle \emph{dense} document text. 

As an alternative, there are a few commercial products designed to handle dense text recognition \cite{gcp_ocr,textract}. We evaluate our method using the public online API of \cite{textract}, results are presented in Table~\ref{tab:comp_textract}. In this case, our model still provides a $5.1\%$ relative improvement. The commercial model \cite{textract} is superior to Tesseract, reducing the mean edit distance from $0.178$ to $0.103$, yet CREASE still maintains a significant gap over DewarpNet of $0.6\%$ absolute and $5.1\%$ relative.

==> tables/e2e.tex <==

\begin{table}[h]
\setlength{\tabcolsep}{6pt}
\centering
\caption{End-to-end Training}
\label{tab:e2e}
\begin{tabular}{lccc}
\hline

          & $E_d$ & EPE & SSIM \\ 
\hline
\hline
No E2E & 0.216	 $\pm$ 0.017 & 0.049 $\pm$ 0.001 & 0.400 $\pm$ 0.005 \\

E2E
  & 0.232 $\pm$ 0.059 & 0.050 $\pm$ 0.003 & 0.400 $\pm$ 0.006 \\
  \hline
E2E Angle
  & 0.204 $\pm$ 0.015 & 0.051 $\pm$ 0.002 & 0.402 $\pm$ 0.005 \\
\hline


\end{tabular}
\end{table}


